OPPO: An Ontology for Describing Fine-Grained Data Practices in Privacy Policies of Online Social Networks

Privacy policies outline the data practices of Online Social Networks (OSN) to comply with privacy regulations such as the EU-GDPR and CCPA. Several ontologies for modeling privacy regulations, policies, and compliance have emerged in recent years. However, they are limited in various ways: (1) they specifically model what is required of privacy policies according to one specific privacy regulation such as GDPR; (2) they provide taxonomies of concepts but are not sufficiently axiomatized to afford automated reasoning with them; and (3) they do not model data practices of privacy policies in sufficient detail to allow assessing the transparency of policies. This paper presents an OWL Ontology for Privacy Policies of OSNs, OPPO, that aims to fill these gaps by formalizing detailed data practices from OSNS' privacy policies. OPPO is grounded in BFO, IAO, OMRSE, and OBI, and its design is guided by the use case of representing and reasoning over the content of OSNs' privacy policies and evaluating policies' transparency in greater detail.

==> ISWC_PARTS.tex <==
\begin{document}
\section{DataItemModule (parts that we decided to exclude from FOIS)}

%Data are what privacy regulations aim to protect and are intrinsically linked to who they are about, that is, the \texttt{DataSubjectRole}, \texttt{DataProviderRole}, and \texttt{DataRecipientRole} that identifies what person or organization is the data about or is sharing and receiving the data. These concepts refine the \texttt{LegalPersonRole} in line with the understanding of roles in BFO \cite{arp2008function}.


 As shown in Figure \ref{fig:datamodule}, \texttt{OPPO:IndividualData} can be anonymous; that is, any personally identifiable information related to an individual is removed, and the processed data remains anonymous -- \texttt{OPPO:AnonymizedData}. OSNs can also collect data, which may directly or indirectly identify an individual's identity -- \texttt{OPPO:PersonalData}-- such as images, fingerprints, posts, reviews, location, and credit card information (financial data).  To distinguish and capture different data types, we introduce 12 categories of data, which are created based on the analysis of GDPR, CCPA, privacy policies, and prior work \cite{gupta2021phin}. Additionally, we reused the concept \texttt{dpvo:InferredPersonalData} from DPV, which may include any new information that is derived from existing data (e.g., demographic information from the browsing history) and can directly or indirectly identify an individual. An OSN can aggregate users' data  using statistical operations --\texttt{OPPO:StatisticalData}-- (e.g., number of views on a product page) or create artificial data to resemble real data --\texttt{dpvo:SyntheticData}.

 Moreover, as mentioned earlier, we identified three roles that are mostly involved while describing an OSN's data practices: (\texttt{OPPO:DataSubjectRole}, \texttt{OPPO:DataRecipientRole}, and \texttt{OPPO:DataProviderRole}). These roles are being distinguished with respect to the relations (\textit{properties}) they have with the \texttt{IAO:DataItem} class. For instance, an human individual may act in the role of \texttt{OPPO:DataSubjectRole}, if the data \texttt{isAbout} the individual. Likewise, an individual's role as \texttt{OPPO:DataRecipientRole} and \texttt{OPPO:DataProviderRole} can be distinguished if the data the \texttt{isRecievedBy} and \texttt{isProvidedBy} by the individual respectively. Furthermore, it is critical to allow that an OSN may have different data practices (\texttt{OPPO:DataPractice}) for different data types. For instance, health-related data may have a different retention period than demographic data. To model this, the data practices (\texttt{OPPO:DataPractice}) are related to the (\texttt{IAO:DataItem}) types using the (\texttt{actsOn}) relation. Similarly, an OSN may employ different security mechanism for different types of data. For example, an organization may apply end-to-end encryption mechanism to biometric data and pseudonamized mechanism to technical data. To capture such detailed data practices, the security mechanisms (\texttt{OPPO:SecurityMechanism}) are related to the \texttt{IAO:DataItem} types using the (\texttt{appliesTo}) relation.



 \section{DataPracticeModule (Parts that have been excluded from FOIS)}

 An OSN's privacy policy (\texttt{OPPO:PrivacyPolicy}) describes (\texttt{hasDataPractice}) the collection, storing, and processing (\texttt{OPPO:DataPractice}) of the users' data. These data practices \texttt{OPPO:DataPractice}) are required to be allowed or disallowed (\texttt{allows/disallows}) by different privacy regulations (\texttt{OPPO:PrivacyRegulation}), followed by the OSN. 

 
\end{document}

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
